Socio-Affective Agents as Models of Human Behaviour in the Networked Prisoner's Dilemma

Affect Control Theory (ACT) is a powerful and general sociological model of human affective interaction. ACT provides an empirically derived mathematical model of culturally shared sentiments as heuristic guides for human decision making. BayesACT, a variant on classical ACT, combines affective reasoning with cognitive (denotative or logical) reasoning as is traditionally found in AI. Bayes\-ACT allows for the creation of agents that are both emotionally guided and goal-directed. In this work, we simulate BayesACT agents in the Iterated Networked Prisoner's Dilemma (INPD), and we show four out of five known properties of human play in INPD are replicated by these socio-affective agents. In particular, we show how the observed human behaviours of network structure invariance, anti-correlation of cooperation and reward, and player type stratification are all clearly emergent properties of the networked BayesACT agents. We further show that decision hyteresis (Moody Conditional Cooperation) is replicated by BayesACT agents in over $2/3$ of the cases we have considered. In contrast, previously used imitation-based agents are only able to replicate one of the five properties. We discuss the implications of these findings in the development of human-agent societies.

==> plot.tex <==
\begin{figure}[tb]
	\centering{
		
		\begin{tikzpicture}[scale=0.7]
		\begin{axis}[
		height=8cm,
		width=11cm,
		grid=major,
		xlabel=Round,
		ylabel=Cooperation Rate,
		legend style={at={(0.5,-0.15)},
			anchor=north,legend columns=3}
		]
		
		%\addplot {-x^5 - 242};
		%\addlegendentry{model}
		
		\addplot+[mark=none,black] table{
			1 0.595
			2 0.53
			4 0.42
			5 0.48
			6 0.42
			7 0.405
			8 0.39
			9 0.42
			10 0.425
			11 0.4
			12 0.42
			14 0.41
			16 0.38
			17 0.39
			19 0.385
			21 0.34
			22 0.39
			24 0.34
			25 0.35
			26 0.345
			28 0.37
			29 0.34
			31 0.36
			32 0.38
			33 0.33
			34 0.34
			35 0.35
			36 0.36
			37 0.36
			38 0.3
			39 0.315
			40 0.375
			41 0.35
			42 0.35
			43 0.31
			44 0.34
			45 0.32
			46 0.31
			47 0.34
			48 0.29
			49 0.275
			50 0.275
			51 0.32
		};
		\addlegendentry{Human}
		
		\addplot+[dashed,mark=none,black] table {
			1 0.5089
			2 0.5148
			3 0.4970
			4 0.4675
			5 0.4675
			6 0.4438
			7 0.5148
			8 0.4793
			9 0.4320
			10 0.4734
			11 0.4793
			12 0.4734
			13 0.4201
			14 0.3609
			15 0.4142
			16 0.4615
			17 0.4260
			18 0.4320
			19 0.4556
			20 0.4675
			21 0.4615
			22 0.4793
			23 0.4379
			24 0.3964
			25 0.5207
			26 0.4201
			27 0.3964
			28 0.3964
			29 0.3905
			30 0.4793
			31 0.4379
			32 0.4320
			33 0.4615
			34 0.4142
			35 0.3964
			36 0.4320
			37 0.4793
			38 0.4320
			39 0.4379
			40 0.4142
			41 0.4675
			42 0.4083
			43 0.4438
			44 0.4201
			45 0.4438
			46 0.4142
			47 0.4497
			48 0.4320
			49 0.3846
			50 0.4320
			51 0.4911
			52 0.4734
			53 0.4615
			54 0.4320
			55 0.4320
			56 0.4201
			57 0.4320
			58 0.4675
			59 0.4379
			60 0.4438
			
		};
		\addlegendentry{BayesACT}
		
		\addplot+[dotted, thick, mark=none,black] table {
			1 0.5562
			2 0.2840
			3 0.1716
			4 0.0888
			5 0.0355
			6 0.0355
			7 0.0178
			8 0.0178
			9 0.0237
			10 0.0118
			11 0.0000
			12 0.0000
			13 0.0000
			14 0.0000
			15 0.0000
			16 0.0000
			17 0.0000
			18 0.0000
			19 0.0000
			20 0.0000
			21 0.0000
			22 0.0000
			23 0.0000
			24 0.0000
			25 0.0000
			26 0.0000
			27 0.0000
			28 0.0000
			29 0.0000
			30 0.0000
			31 0.0000
			32 0.0000
			33 0.0000
			34 0.0000
			35 0.0000
			36 0.0000
			37 0.0000
			38 0.0000
			39 0.0000
			40 0.0000
			41 0.0000
			42 0.0000
			43 0.0000
			44 0.0000
			45 0.0000
			46 0.0000
			47 0.0000
			48 0.0000
			49 0.0000
			50 0.0000
			51 0.0000
			52 0.0000
			53 0.0000
			54 0.0000
			55 0.0000
			56 0.0000
			57 0.0000
			58 0.0000
			59 0.0000
			60 0.0000
			
		};
		\addlegendentry{Imitator}
		
		\addplot+[dashed,mark=none,black] table {
			1 0.6627
			2 0.7337
			3 0.7396
			4 0.6864
			5 0.7160
			6 0.7041
			7 0.7515
			8 0.7041
			9 0.7396
			10 0.7278
			11 0.7278
			12 0.6864
			13 0.6746
			14 0.6568
			15 0.6331
			16 0.6805
			17 0.6982
			18 0.6923
			19 0.6272
			20 0.7101
			21 0.6982
			22 0.7041
			23 0.6331
			24 0.7219
			25 0.6509
			26 0.6686
			27 0.6391
			28 0.6686
			29 0.7456
			30 0.6805
			31 0.7041
			32 0.6982
			33 0.7160
			34 0.6864
			35 0.6805
			36 0.6686
			37 0.7396
			38 0.7160
			39 0.6686
			40 0.7456
			41 0.6627
			42 0.7219
			43 0.6627
			44 0.6746
			45 0.6805
			46 0.7041
			47 0.7219
			48 0.7574
			49 0.6982
			50 0.6746
			51 0.6686
			52 0.7160
			53 0.6982
			54 0.6982
			55 0.7101
			56 0.7041
			57 0.7041
			58 0.6213
			59 0.7692
			60 0.7278
			
		};
		%\addlegendentry{BayesACT}
		
		\addplot+[dotted, thick, mark=none,black] table {
			1 0.4320
			2 0.4379
			3 0.4142
			4 0.4083
			5 0.4142
			6 0.4083
			7 0.4320
			8 0.4201
			9 0.4201
			10 0.4675
			11 0.4260
			12 0.4024
			13 0.4320
			14 0.5030
			15 0.5266
			16 0.5030
			17 0.5680
			18 0.5858
			19 0.5503
			20 0.5444
			21 0.5266
			22 0.6272
			23 0.6213
			24 0.5740
			25 0.5503
			26 0.5207
			27 0.5503
			28 0.5621
			29 0.5503
			30 0.5799
			31 0.6213
			32 0.6213
			33 0.6331
			34 0.6450
			35 0.6509
			36 0.7219
			37 0.7456
			38 0.7811
			39 0.8107
			40 0.8521
			41 0.8639
			42 0.8580
			43 0.8462
			44 0.8580
			45 0.8639
			46 0.9112
			47 0.9290
			48 0.9408
			49 0.9290
			50 0.9408
			51 0.9408
			52 0.9112
			53 0.9112
			54 0.8876
			55 0.8935
			56 0.9112
			57 0.8817
			58 0.9231
			59 0.9231
			60 0.9053
		};
		%\addlegendentry{Imitator}
		
		\end{axis}
		\end{tikzpicture}
		
		\caption{\label{fig:coopRates} Cooperation rates by round for human players~\protect\cite{gracia2012heterogeneous} (which had matrix parameters $T=10, R=7, P=0, S=0$, and used a grid layout with a von Neumann neighbourhood)~\protect\cite{gracia2012heterogeneous}, and selected simulations for BayesACT (bottom: BACTD1/M2/ER8, top: BACTS0/M1/Grid) and imitator (bottom: IM50/M2/Grid, top: IM100/M3/Grid) agents.}
	}
\end{figure}

